Learning Emergence of Interaction Patterns across Independent RL Agents in Multi-Agent Environments

Many real-world problems, such as controlling swarms of drones and urban traffic, naturally lend themselves to modeling as multi-agent reinforcement learning (RL) problems. However, existing multi-agent RL methods often suffer from scalability challenges, primarily due to the introduction of communication among agents. Consequently, a key challenge lies in adapting the success of deep learning in single-agent RL to the multi-agent setting. In response to this challenge, we propose an approach that fundamentally reimagines multi-agent environments. Unlike conventional methods that model each agent individually with separate networks, our approach, the Bottom Up Network (BUN), adopts a unique perspective. BUN treats the collective of multi-agents as a unified entity while employing a specialized weight initialization strategy that promotes independent learning. Furthermore, we dynamically establish connections among agents using gradient information, enabling coordination when necessary while maintaining these connections as limited and sparse to effectively manage the computational budget. Our extensive empirical evaluations across a variety of cooperative multi-agent scenarios, including tasks such as cooperative navigation and traffic control, consistently demonstrate BUN's superiority over baseline methods with substantially reduced computational costs.

==> extra.tex <==
\begin{table*} \label{TrafficTable}
\caption{}
% and the reason for excluding the reward for 8 agents with the weights trained on 14 agents is to increase the number of agents to test scalability but not to decrease
\label{swarm}
\vskip 0.15in
\begin{center}
\begin{small}
\begin{sc}
\begin{tabular}{l|c|cc|cc||c|cc|cc|}
\toprule
&\multicolumn{5}{c}{Grid 2$\times$2}&\multicolumn{5}{c}{Inglodast Corridor}\\
&\multicolumn{1}{c}{FLOPS}&\multicolumn{2}{c}{Avg. Wait}&\multicolumn{2}{c}{Avg. Trip Time}&\multicolumn{1}{c}{FLOPS}&\multicolumn{2}{c}{Avg. Wait}&\multicolumn{2}{c}{Avg. Trip Time}\\
\midrule
Model& FLOPS& Train & Test& Train & Test & FLOPS& Train & Test & Train & Test\\
\hline
Centralized & 2.6$e$6$(1x)$&2.41 &2.08 & 69.61&67.93 & 7.5$e$6$(1x)$&12.53&  &74.00  &\\
 Decentralized & 6.6$e$5$(0.25x)$&3.96 &3.29 & 71.75&69.03 &1$e$6$(0.14x)$&15.87&  &  77.36&\\
 BUN &6.6$e$5$(0.25x)$ &2.25 &1.96 & 69.35& 67.52&1$e$6$(0.14x)$ &12.42&  & 73.86 &\\
 RigL &6.6$e$5$(0.25x)$ &2.39 &2.01 & 69.38&67.72& 1$e$6$(0.14x)$&13.83&  & 76.27 &\\
  \bottomrule
%14 Agents & 1 & 1 & 1 & 1\\
\end{tabular}
\end{sc}
\end{small}
\end{center}
\vskip -0.1in
\end{table*}
